Unified Graph Structured Models for Video Understanding

Accurate video understanding involves reasoning about the relationships between actors, objects and their environment, often over long temporal intervals. In this paper, we propose a message passing graph neural network that explicitly models these spatio-temporal relations and can use explicit representations of objects, when supervision is available, and implicit representations otherwise. Our formulation generalises previous structured models for video understanding, and allows us to study how different design choices in graph structure and representation affect the model's performance. We demonstrate our method on two different tasks requiring relational reasoning in videos -- spatio-temporal action detection on AVA and UCF101-24, and video scene graph classification on the recent Action Genome dataset -- and achieve state-of-the-art results on all three datasets. Furthermore, we show quantitatively and qualitatively how our method is able to more effectively model relationships between relevant entities in the scene.

==> tables/computational_complexity.tex <==


\begin{table*}[t]
	\centering
	\caption{Compute used by baseline and proposed models.
				 Our graph model is significantly more efficient than Non-local in the last layer of the backbone as it only passes messages to actor nodes, instead of all elements in the feature map.
				 Computation increases linearly with the number of frames processed, (and thus $\tau_c$), as the majority of compute is performed by the ResNet backbone.	
}
	\begin{tabular}{lcccc}
		\toprule
		Model & Frames & GFLOPs & Parameters ($\times10^6$) & SGCls R@20 \\ 
		\midrule
		SlowFast (ResNet 50)            						 & 32 &   74.18        &   34.6    &  48.9   \\
		Non-local in backbone           		  			   & 32 &   83.66         &   43.0    &  49.1   \\
		\midrule
		Spatial model, GAT, $\tau_c = 1$       		      & 32 &   74.41        &   36.5    & 51.1  \\
		Spatial model, Non-local, $\tau_c = 1$ 	        & 32 &   74.47        &   37.0    & 50.4 \\
		\midrule
		Spatio-temporal, GAT, $\tau_c = 3$     	        & 96   &   223.25      &   36.5   & 53.5  \\ 
		Spatio-temporal, GAT, $\tau_c = 5$     	        & 160 &   372.08      &   36.5   & 53.8  \\ 
		\bottomrule
	\end{tabular}
	\label{tab:compute}
\end{table*}
